Significance of Low-level Controller for String Stability under Adaptive Cruise Control

Current commercial adaptive cruise control (ACC) systems consist of an upper-level planner controller that decides the optimal trajectory that should be followed, and a low-level controller in charge of sending the gas/brake signals to the mechanical system to actually move the vehicle. We find that the low-level controller has a significant impact on the string stability (SS) even if the planner is string stable: (i) a slow controller deteriorates the SS, (ii) slow controllers are common as they arise from insufficient control gains, from a "weak" gas/brake system or both, and (iii) the integral term in a slow controller causes undesired overshooting which affects the SS. Accordingly, we suggest tuning up the proportional/feedforward gain and ensuring the gas/brake is not "weak". The study results are validated both numerically and empirically with data from commercial cars.

==> good_deletes.tex <==

% \subsubsection{Impact of measurement noise}
% In this simulation, we run the combination of linear planner and PID controller under the influence of speed and position measurement noise $n_x \sim \mathcal{N}(0,\, 0.25)$ and $n_v \sim \mathcal{N}(0,\, 0.04)$. As mentioned before, increasing P gain can help the controller respond faster and improve SS, however, high P gain can also amplify the noise in the system, further jeopardizing SS (as shown in Fig. in \ref{NosieACC}, the original SS in a noise-free environment is compromised after noise is included). Moreover, the noise can also induce choppy accelerations (the choppyness is further exacerbated under high control gains), which significantly compromises riding comfort and vehicle actuators.

% Therefore, a decent performance of vehicle state estimation and measurement filtering are of great significance for the real-word implementation. The smooth measurement can not only benefit riding comfort, but also enhance SS performance. In the Openpilot, the measurement filtering and trajectory smoothing are embedded in the longitudinal control system, which enable us to circumscribe the adversaries of noise, and validate the SS performance (will be demonstrated in the following section).

% \begin{figure}[htbp]
% \centering
% \begin{subfigure}[t]{0.4\linewidth}
%     \includegraphics[width=\linewidth]{PI/ACCPID_noNoise.png}
%     \caption{Noise-free case}
% \end{subfigure}%
% \begin{subfigure}[t]{0.4\linewidth}
%     \includegraphics[width=\linewidth]{PI/ACCPID_Noise.png}
%     \caption{Case with measurement noise}
% \end{subfigure}%
%     \caption{Impact of measurement noise}
%     \label{NosieACC}
% \end{figure}


% Unfortunately, the current short answer is no. This study specifically points out that the gap between SS theory and practice lies in the impact of low-level controller, which has been consistently neglected so far. We argue that, any design of ACC planner without a low-level controller is incomplete, since how well the planned trajectory can be executed will remain unknown. We provide evidence to the argument by realizing some underlying issues in the previous experiments with the low-level controller applied. Specifically, in the ACC design experiments of existing literature, researchers used either original equipment manufacturer (OEM) controller applied in the factory ACC system or in-house designed controller. The OEM controller \citep{Eilbert2020PerformanceCO} directly tracks the acceleration/speed command, or torque/brake pressure generated from the upper-level planner to realize ACC functionality. However, the algorithms of OEM controllers are unclear and difficult to analyze due to its 'black-box' property.
% The in-house designed controllers are developed through directly accessing the vehicle engine/brake control units, which apply specific feedback control law to supply setpoints to the engine/brake control units for achieving desired tracking of planned trajectories. For instances, \cite{naus2010string,6082981} used a MOVE gateway to interact with the vehicle motor to achieve decent acceleration setpoint tracking performance. \cite{Lu2018TruckCS} applied feedback linearization control to calculate the desired torque/brake pressure command of truck actuators to achieve desired tracking of planned acceleration. \cite{Shladover2009EffectsOC} utilized the loop-shaping techniques to devise a speed servo to track the planned speed. The in-house designed controllers demonstrated desired performance in the experiment. However, they are only applied to specific filed-test scenarios and serve for specific performance index, it's unclear if in-house designed controllers still perform in a decent way in the real-world driving (which involves more objectives such as comfort, product longevity, and fuel economy). Additionally, most in-house designed controllers are not open-sourced for further research usage or testing.



% have:
% \begin{align}
%     e(n) \approx  (1-k_p dt)v_{\text{pid}}(n)
%     \label{approx-p-error}
% \end{align}
% Consequently,  we can notice 
% a slow controller (with smaller $k_p$) will lead to larger tracking error $e(n)$ at each step.

% The maximum integral accumulation $\mathcal{I}$ during the rise of the oscillation is:
% \begin{align}
%     \mathcal{I}& = (1-k_p dt) \Sigma_{n=T}^{T+\Delta T_e} v_{\text{pid}}(n)
%     \label{over-value}
% \end{align}
% \begin{align}
%     \mathcal{I}& = \Sigma_{n=T}^{T+\Delta T_e} [-(1+k_p dt)(1-k_p dt)^{n} v_{ego}(0) - \Sigma_{i=1} ^{n-1} (k_p dt) (1-k_p dt)^{n-i} v_{\text{pid}}(i) + (1-k_p dt)v_{\text{pid}}(n)]
%     \label{over-value}
% \end{align}
% \begin{align}
%     \mathcal{I}& = \Sigma_{n=T}^{T+\Delta T_e} e(n)  \\
%     & \approx k_p \Delta V_{ov} \label{over-value}
% \end{align}
% where $\Delta V_{ov}$ is the overshooting speed that cancels out the integral accumulation.



% recalling that $v_{pid}(0) = v_{ego}(0)$ and 
% combining it with \eqref{dynamics-pid}, we can derive $v_{ego}(n)$ at time step $n$ in terms of the independent variable $v_{pid}$ and P gain $k_p$:
% \begin{equation}
%     v_{ego} (n) = v_{ego}(t_0) + \Sigma_{1}^n (k_p dt) (1-k_p dt)^{n-1-i} v_{\text{pid}}(i) % \quad \text{for} \quad i=1,2,...,N-1
%     \label{P-impact}
% \end{equation}
%\begin{equation}
    %v_{ego}(n) = (1+k_p dt) (1-k_p dt)^{n} %v_{ego}(0) + \Sigma_{i=1} ^n (k_p dt) %(1-k_p dt)^{n-i} v_{\text{pid}}(i)\quad %\text{for} \quad i=1,2,...,n-1
%    \label{P-impact}
%\end{equation}
%Then the tracking error $e(n)=v_{pid}(n)-v_{ego}(n)$ at time step $n$ can be derived:
% \begin{align}
%     e(n) =  v_{ego}(t_0) + \Sigma_{1}^n (k_p dt) (1-k_p dt)^{n-1-i} v_{\text{pid}}(i)
% \end{align}



% Noticing that at time $T+\Delta T$, \eqref{v_{\text{target}}_rate} should be equal to zero due to the stable point, thus we have:  

% \begin{align}
%     k v_{\text{rel}}(T+\Delta T)& = -(1-k  \tau) a_{\text{lead}}(T+\Delta T)\\
%     v_{\text{rel}}(T+\Delta T) & = - \frac{1-k  \tau}{k} a_{\text{lead}}(T+\Delta T)\\
%     v_{\text{ego}}(T+\Delta T) & = v_{\text{lead}}(T+\Delta T)+\frac{1-k  \tau}{k} a_{\text{lead}}(T+\Delta T)
%     \label{getTDeltaT}
% \end{align}


% For either speed increase or decrease, we can have a unified formula as:
% \begin{equation}
%     \Delta v_{\text{target}} = k \sum_{T_1\le \hat{t} \le T_1+\Delta T} v_{\text{rel}}(\hat{t}) + (1-k  \tau) \overline{a}_{lead} \Delta T
%     \label{v_{\text{ego}}_impact}
% \end{equation}

%To evaluate the follower speed amplification magnitude

==> recycle.tex <==
% \begin{align}
%     \Delta vStart &=\int_{T}^{T+\Delta T} \dot{vStart} (\tau) d\tau\\
%     &= 0.5 \int_{T}^{T+\Delta T} (aTarget(\tau) + aStart(\tau)) d\tau \\
%     & = 0.5
%     \label{vStart-integral}
% \end{align}

% \begin{align}
%     |\Delta vStart| &= |vStart(T+\Delta T) - vStart(T)|\\
%     & = 0.5 T_{s} \sum_{\hat{t} \in [0, T+\Delta T]} |aTarget(\hat{t}) + aStart(\hat{t})|
% \intertext{if $T_{s}=T_{p}$, we have:}
% |\Delta vStart| & = T_{s} \sum_{\hat{t} \in [0, T+\Delta T]} |aTarget(\hat{t})|
% \label{vStart-integral}
% \end{align}


% Similar mechanism can be found for the F-only controller and thus hold for a P+F controller as well. In the following section we will show that an integral term can sometimes be opposite to the proportional and feedforward control, which makes the controller slower.   


% For a PIF controller, there exist different methods to compute the low-level $vPid$ and $aPid$ using the merely $aTarget(\hat{t})$, $vTarget(\hat{t})$ or both of them. In order to make the upper-planner independent, the update of $vPid$ and $aPid$ are expected to work independently from the noisy vehicle responses such as $aEgo$ or $vEgo$. Thus it is common to introduce surrogate variables in planner, for example, $aStart$ and $vStart$ are often used to replace $aEgo$ and $vEgo$ when computing those low-level setpoints $aPid$ and $vPid$. 


% Taking the derivative of \eqref{aStart-vStart}, we have:
% \begin{align}
%     \dot{aStart} &= (aTarget-aStart)/T_p  \\
%     \dot{vStart} &= (aTarget + aStart)/2
%     \label{mpc-planner}
% \end{align}


% \begin{equation}
%     \Delta vTarget \propto k_v \int_{T_1}^{T_1+\Delta T} |vRel| dt
%     \label{vEgo_impact}
% \end{equation}


% Taking the second derivative of $\Delta vTarget$ leads to:

% \begin{equation}
%     \dot{|\Delta vTarget|} = |aEgo| \approx k_p \cdot e + k_i \cdot \int_{0}^t {e} +k_f \cdot aPid
%     \label{control_analysis}
% \end{equation}



% From now on, we omit the index $\hat{t}$ for $vStart$, $aStart$ and $aTarget$, and use $dt$ to denote the elapsed time from the most recent planning time $\hat{t}$.

% The low-level setpoints given a MPC upper-planner can be computed as:
% \begin{align}
%     aPid(dt) & = aStart + dt \frac{ aTarget-aStart}{T_{mpc}}  \\
%     vPid(dt) & = vStart + dt \frac{aPid(dt) + aStart}{2}
% \end{align}

% Here $aTarget$ is calculated by the MPC palnner with a step length $T_{mpc}$. Note that $aStart$ and $vStart$ are initialized using $aEgo$ and $vEgo$, but one can expect the accumulating errors between them because the planner is running independently. 


% The feedforward control for $\hat{t}+dt$ is:
% \begin{align}
%      k_f \cdot aPid(\hat{t}+dt) = k_f [aStart +  \frac{dt(aTarget-aStart) }{T_{mpc}}]
%      \label{mpc-f}
% \end{align}

% At time $\hat{t}+dt$, the proportional term $k_p \cdot e$ is:

% \begin{align}
% k_p \cdot e = & k_p [(vStart + \frac{dt}{2} (2aStart + \frac{dt(aTarget-aStart)}{T_{mpc}}) \nonumber \\
% &-vEgo] 
% \label{mpc-p}
% \end{align}

% From \eqref{mpc-f} and \eqref{mpc-p}, we see the P and F control inputs both depend on $vStart$ and $aStart$, which are prone to cumulative errors because they are totally independent of the low-level controller and responses. 


% To understand the impact of low-level controller, in this study, we use an after-market self-driving device, Comma Two, to test out customized ACC on real vehicle, because Comma Two allows users to run a customized Openpilot \cite{openpilot} program to replaces the stock ACC modules from the original equipment manufacturer, which provides us with flexibility to control the vehicle using our own algorithm. Specifically, we analytically and experimentally analyze the impacts of time headway, and sensitivity parameter of the high-level planner, and the control gains of the low-level controller, on the tracking performance (e.g., overshooting and undershooting issues, decay of tracking error, etc.) of reference speed.



\begin{comment}
The study bases its theory, tests and analysis on the open-source ACC system in Openpilot, Comma.ai. Two types of longitudinal control algorithms have been introduced, which are a linear planner with a PI controller and an MPC planner followed by a PIF controller. For both longitudinal control pipelines, we achieved the same findings regarding the low-level controller's impact. The influence of high-level planners is out of the scope for this paper and has not been fully studied. In literature the linear planner is assumed to have a constant parameter, while in practice it is often interpolated by speed values. 
\end{comment}

% \subsection{High-level planner}
% To study the underlying mechanisms, it is necessary to first introduce the high-level planner considering the coupled effect. 
% Unfortunately, for a non-linear MPC planner, the  dynamics of $aTarget$ in \eqref{mpc-planner} is difficult be to explicitly obtained like \eqref{vTarget} for a linear-type controller, in that the constrained MPC foils the tractability of the problem.


% \begin{enumerate}
% \item  Introducing all variables and constants: i) set up the current state variables including current speed, acceleration and position; and ii) estimate lead vehicle position and speed for the simulation horizon, use them as online data. 
% \item set up the car ODE model
% \item set up a least-square objective function by defining the cost function consisting of four aspects (time to collision, distance, acceleration and jerk) and the weighting matrix. 
% \item Defining a complete optimal control problem comprising the dynamic model, the objective function as well as constraints on the input.
% \item Setting up a real-time algorithm defined by the OCP to be solved at each sampling instant together with a sampling time specifying the time lag between two sampling instants.
% \item Setting up a controller by specifying a control law, i.e. the real-time algorithm solving our OCP in this case, and a reference trajectory to be tracked. 
% \item return the solution
% \end{enumerate}


\begin{comment}
\author{\IEEEauthorblockN{1\textsuperscript{st} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{4\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
}
\end{comment}





\begin{align}
    \Delta v_{target} & = v_{target}(T_1+\Delta T)- v_{target}(T_1) \nonumber \\
    & = \sum_{T_1\le \hat{t} \le T_1+\Delta T} k_v (v_{lead}(\hat{t})-v_{ego}(\hat{t})) dt \nonumber  \\
    &+ \sum_{T_1\le \hat{t} \le T_1+\Delta T}(1-k_v  H_t) a_{lead}(\hat{t}) dt \nonumber \\
    & = k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} vRel(\hat{t}) + (1-k_v  H_t) \overline{a_{lead}} \Delta T
    \label{analysis}
\end{align}
where $\overline{a_{lead}}$ is the average acceleration for the lead vehicle from in $\Delta T$. Obviously $v_{lead}$ and $a_{lead}$ do not change with the follower, thus the magnitude of the speed change for the ego vehicle will only depend on $vRel$. Also notice that $1-k_v H_t>0$ for common values. For either speed increase or decrease, we can have a unified formula as:

\begin{equation}
    |\Delta v_{target}| = k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} |vRel(\hat{t})| + (1-k_v  H_t) |\overline{a_{lead}}| \Delta T
    \label{v_{ego}_impact}
\end{equation}

Subtract the lead vehicle speed change during $\Delta T$, we derive the SS index $I_{linear}$ to denote the speed amplification:
\begin{align}
   I_{linear} = &|\Delta v_{target}|-|\Delta v_{lead}|\nonumber \\
   & = k_v (\sum_{T_1\le \hat{t} \le T_1+\Delta T} |vRel(\hat{t})| - H_t |\overline{a_{lead}}| \Delta T)
    \label{SS-index-ACC}
\end{align}
where $I_{linear} \geq 0$, and larger values indicate more amplification in follower's speed and worse SS.


% Similarly, we can have an index $I_{mpc}$ to denote the speed amplification with a MPC controller:

% \begin{align}
% \frac{2}{T_s} I_{mpc} = & \frac{2}{T_s} |\Delta v_{start}-\Delta v_{lead}| \nonumber \\ &= \sum_{T_1\le \hat{t} \le T_1+\Delta T} |a_{target}(\hat{t}) \nonumber \\
% & + \sum_{n = 0} ^{\hat{t}} \frac{Ts}{Tp} (1-\frac{Ts}{Tp})^{\hat{t}-1-n} a_{target}(n)|
% \label{SS-a_{target}}
% \end{align}


% This section we will release the assumption of mapping function from gas/brake to acceleration, since on most cars it is unknown and potentially complex than a scale factor. First we present the results using some virtual cars with unknown dynamics in the self-driving vehicle simulator, Carla. It allows us to repeat the platoon experiments with little cost. In addition, we tried to verify our major findings using real cars with only a human-driven lead vehicle and a ACC-equipped vehicles with the same control algorithm used above. 

% \subsection{Carla experiments of platoons}
%  To derive the compute\_gb function, we applied constant gas/brake value to a Tesla Model 3 (with one gear) in Carla, and fit the curves between speed and acceleration values at different gas/brake levels; see Fig.\ref{Carla_gb}. 
 
%  \begin{figure}
%      \centering
%      \includegraphics[width=\linewidth]{carla_gb.png}
%      \caption{Relationship between gb and acceleration in Carla}
%      \label{Carla_gb}
%  \end{figure}

% Note that the linear model is a reasonable fit and this is also supported by the linear relationship between speed and accelerations found in literature collecting human drives \citep{}.



_____________________


% Consider that the proportional gain has a dominant effect, and in discrete-time implementation the integral gain and derivative gain can all be converted into proportional gain, we omit the integral and derivative term for now:

% \begin{equation}
%      a_{ego} = control \approx k_p  (v_{pid}-v_{ego})
%      \label{P-dynamics}
% \end{equation}

For a linear planner as shown in \eqref{desire_d} and \eqref{ACC-vt}, it satisfies:
\begin{equation}
\begin{aligned}
    \dot{s}_{ego} & = v_{lead} - v_{ego} \\
    \dot{s}_{des} &=  \tau \dot{v}_{lead} \\ 
    \dot{v}_{lead} & = a_{lead}
    \label{ACC}
\end{aligned}
\end{equation}

Substituting \eqref{ACC} into \eqref{ACC-vt}, we have: 
\begin{equation}
    \dot{v}_{target} = k_v (v_{lead}-v_{ego}) + (1-k_v  \tau) a_{lead}
    \label{vt_rate}
\end{equation}

To investigate the impact on SS, we evaluate the maximum changes in the ego vehicle target speed, namely $\Delta \vt$, which can be calculated by tracking \eqref{vt_rate} from the time $T_1$ when the ego car starts to react to the lead vehicle, to the time $T_1+\Delta T$ when the ego car starts to reduce the overshoot/undershoot (see Fig.\ref{undershooting_actuator}(e)):
\begin{align}
    \Delta \vt & = \vt(T_1+\Delta T)- \vt(T_1) \nonumber \\
    & = \sum_{T_1\le \hat{t} \le T_1+\Delta T} k_v (v_{lead}(\hat{t})-v_{ego}(\hat{t})) d\hat{t} + (1-k_v  \tau) a_{lead}(\hat{t}) d\hat{t} \nonumber \\
    % & =  (1-k_v  \tau) \overline{a}_{lead} \Delta T + k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} v_{rel}(\hat{t}) d\hat{t}
    & = (1-k_v  \tau) \overline{a}_{lead} \Delta T + k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} (v_{lead}(\hat{t})-\vt(\hat{t}-d\hat{t}))  d\hat{t} + k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} (\vt(\hat{t}-d\hat{t}) - v_{ego}(\hat{t}))d\hat{t} \nonumber \\
    % & = (1-k_v  \tau) \overline{a}_{lead} \Delta T + k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} v_{lead}(\hat{t})d\hat{t} - k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} \vt(\hat{t}) d\hat{t}+ k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} (\vt(\hat{t}-d\hat{t}) - v_{ego}(\hat{t}))d\hat{t} \\
    & = (1-k_v  \tau) \overline{a}_{lead} \Delta T + k_v  \overline{v}_{lead} \Delta T - k_v \overline{v}_{target} \Delta T+ k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} (\vt(\hat{t}-d\hat{t}) - v_{ego}(\hat{t}))d\hat{t}
    \label{analysis}
\end{align}
where $\overline{a}_{lead}$, $\overline{v}_{lead}$ and \textbf{$\overline{v}_{target}$}, are the average acceleration,speed for the lead vehicle and mean target speed for the follower respectively during $\Delta T$. Also notice that $1-k_v \tau>0$ for rational values of the gain $k_v$ and desired time headway $\tau$. 

% Since $v_{lead}$ and $a_{lead}$ do not change with the follower, the magnitude of the perturbation for the ego vehicle will only depend on relative speed $v_{rel}$.

Further, define the tracking error $e_t$ as the speed difference in the low-level controller and the given target speed from planner. For each planning period $[\hat{t}, \hat{t}+d\hat{t}]$, we have:
\begin{equation}
    e_t (\hat{t}) =  \vt(\hat{t})-v_{ego}(\hat{t}+d\hat{t}) =  \vt(\hat{t})-v_{ego}(\hat{t}) - d\hat{t} \cdot \Bar{a}_{ego}(\hat{t}) 
    \label{tracking_error}
\end{equation}
where $\Bar{a}_{ego}(\hat{t})$ is the average acceleration in one planning period.


Substituting \eqref{tracking_error} into \eqref{analysis}, we have:
\begin{equation}
    \Delta \vt =  (1-k_v  \tau) \overline{a}_{lead} \Delta T + k_v  \overline{v}_{lead} \Delta T - k_v \overline{v}_{target} \Delta T+k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} e_t(\hat{t})  d\hat{t}
    % (1-k_v  \tau) \overline{a}_{lead} \Delta T + k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} v_{rel} ^{target} (\hat{t})  d\hat{t} + k_v \sum_{T_1\le \hat{t} \le T_1+\Delta T} e_t(\hat{t})  d\hat{t}
\end{equation}
% where $v_{rel} ^{target} (\hat{t}) = v_{lead}(\hat{t})-\vt(\hat{t})$.

To evaluate the speed amplification of the follower, we subtract the lead vehicle speed change $\Delta v_{lead}$ during $\Delta T$, which defines the SS index $I_{linear}$ for acceleration or deceleration:
\begin{align}
   I_{linear} = & \frac{|\Delta \vt|-|\Delta v_{lead}|}{|\Delta v_{lead}|} \nonumber \\
%   & = k_v (\frac{\sum_{T_1\le \hat{t} \le T_1+\Delta T} |v_{rel}(\hat{t})|}{|\Delta v_{lead}|}- \tau) \nonumber \\
   & = -k_v \tau + k_v \frac{\overline{v}_{lead} - \overline{v}_{target} + \Bar{e}_t}{|\Delta v_{lead}|/\Delta T} \nonumber \\
   & = -k_v \tau + k_v \frac{k_v }{|\Bar{a}_{lead}|} + k_v \frac{\Bar{e}_t}{|\Bar{a}_{lead}|}
%   & = k_v (\frac{|\Bar{v}_{rel} ^{target}| + |\Bar{e}_t| }{|\Bar{a}_{lead}|}-\tau) \\
%   & = k_v (\frac{|\Bar{v}_{rel} ^{target}| }{|\Bar{a}_{lead}|}-\tau) + k_v \frac{|\Bar{e}_t| }{|\Bar{a}_{lead}|}
    \label{SS-index-ACC}
\end{align}
where $\Bar{v}_{rel} ^{target}$ is the average relative speed given by the planner, and $\Bar{e}_t$ is the average speed tracking error during $\Delta T$. 


% k_v (\frac{|\Bar{v}_{rel} ^{target}| }{|\Bar{a}_{lead}|}-\tau) + k_v \frac{|\Bar{e}_t| }{|\Bar{a}_{lead}|}

A smaller $I_{linear}$ is desirable as it corresponds to better SS. If $I_{linear} > 0$ the speed change is amplified from leader to the follower, yielding a string unstable case. \eqref{SS-index-ACC} suggests the SS is affected by both of the planner and the low-level controller via $\Bar{v}_{rel} ^{target}$ and $\Bar{e}_t$ respectively. Unfortunately, those two components are not independent: the tracking error $e_t(\hat{t})$ of low-level controller for current cycle $\hat{t}$, will cause the planner to compensate at next cycle, i.e.  induces a larger desired speed $\vt(\hat{t}+1)$, if the error is $e_t(\hat{t})$ greater. Note that this is a nice property that help circumvent the complex coupling effect, because larger $e_t(\hat{t})$ lead to larger $\Bar{v}_{rel} ^{target}$. Then we just need to focus on the tracking error in low-level controller.

From \eqref{tracking_error}, the average tracking error in single planning period can be estimated as:
\begin{equation}
    \Bar{e}_t(\hat{t})  = | \vt(\hat{t})-v_{ego}(\hat{t})|/d\hat{t}  -\Bar{a}_{ego}(\hat{t}) 
    \label{avg-tracking_error}
\end{equation}

For a PI controller, considering the dominant impact of P gain, we can approximate $a_{ego} \approx k_p  (v_{pid}-v_{ego})$. Then, assuming an optimal P gain $k^*_p$ happens to reduce the average tracking error $\Bar{e}_t(\hat{t})$  in \eqref{avg-tracking_error} to zero, we have:
% we can approximate the average $\Bar{a}_{ego}$ in single planning period as:
\begin{align}
    \Bar{a}_{ego}(\hat{t})  = (\vt(\hat{t})-v_{ego}(\hat{t}))/d\hat{t} 
    % \propto k_p^* \overline{v_{pid}-v_{ego}}
    \label{origin_controller}
\end{align}


For simplicity, we assume the tracking error in one planning cycle is linearly proportional to the true P gain $\beta k_p^*$ ($0<\beta<1$) in the low-level controller. Then we have :
\begin{align}
        |e_t(\hat{t})|  \approx (1-\beta) |\vt(\hat{t})-v_{ego}(\hat{t})| \label{error-single-linear}
\end{align}

Therefore, a slower controller ($0<\beta<1$) exerts negative impact on SS, as it will make the tracking error $\Bar{e}_t$ become larger and take longer time to decay. For a faster controller ($\beta>1$), the tracking error is more likely close to 0, because the controller can even move to the target speed more quickly due to the excessive gas/brake values; see Algorithm 1. However, for too large P gain, undesired oscillations will occur which makes speed unstable. 


% can have large value in a planning period, indicating undesired fluctuations which undermines SS.

% However, it can also be shown that excessively large control gain will also exert negative impact on SS. 



%Then the discounted P gain $\beta k_p^*$ would lead to the tracking error in single planning period:
% Then we apply the enlarged P gain $\beta k_p^*$, $\beta>1$, to investigate the evolution of tracking error in a single planning period:

% We can see that for an excessive P gain ($\beta>1$), the tracking error can have large value in a planning period, indicating undesired fluctuations which undermines SS.

% \begin{align}
%         |e_t(\hat{t})| & = |\vt(\hat{t})-v_{ego}(\hat{t}+d\hat{t})| - \Bar{a}_{ego} \cdot d\hat{t}  \nonumber \\
%          & \approx |\vt(\hat{t})-v_{ego}(\hat{t})| - \beta |\vt(\hat{t})-v_{ego}(\hat{t})|  \nonumber \\
%         & \approx (1-\beta) |\vt(\hat{t})-v_{ego}(\hat{t})| \label{error-single-linear}
% \end{align}



%where $0<\beta<1$ and smaller $\beta$ indicates a slower PI controller. For $\beta>1$, excessive P gain may cause fluctuations. 
% we can notice the adversarial impact of a slow low-level controller, as it takes longer time for the speed tracking error $e$ to decay, which will induce larger value of $I_{linear}$, amplifying the speed fluctuations.

% Notice when the tracking error in \eqref{tracking_error} is zero, it indicates $\Bar{a}_{ego} = |\vt(\hat{t})-v_{ego}(\hat{t})|/d\hat{t} $

% Substitute the approximated low-level dynamics \eqref{origin_controller} into the tracking error \eqref{tracking_error}, and assume the  we have:
% \begin{align}
%         |e_t(\hat{t})| & =  |\vt(\hat{t})-v_{ego}(\hat{t}+d\hat{t})|  \nonumber \\
%          & \approx |\vt(\hat{t})-v_{ego}(\hat{t})| - k_p |\vt(\hat{t})-v_{ego}(\hat{t})| \quad \text{for} \quad t \in \{\hat{t},\hat{t}+dt,... \hat{t}+d\hat{t}\} \nonumber \\
%         & \approx (1-k_p) |\vt(\hat{t})-v_{ego}(\hat{t})|
% \end{align}
% \begin{align}
%         |e_t(\hat{t})| & =  |\vt(\hat{t})-v_{ego}(\hat{t}+d\hat{t})|  \nonumber \\
%         %  & = |\vt(\hat{t})-v_{ego}(\hat{t})|- d\hat{t} \cdot |\Bar{a}_{ego}(t)| \quad \text{for} \quad t \in \{\hat{t},\hat{t}+dt,... \hat{t}+d\hat{t}\} \nonumber \\
%           & \approx |\vt(\hat{t})-v_{ego}(\hat{t})| - \Sigma_t |v_{ego}(t) - v_{pid}(t)| \quad \text{for} \quad t \in \{\hat{t},\hat{t}+dt,... \hat{t}+d\hat{t}\} \nonumber \\
%         & \approx (1-k_p) |\vt(\hat{t})-v_{ego}(\hat{t})|
% \end{align}


% \begin{equation}
%     \Bar{e} \approx \frac{a_{ego}}{k_p} \label{p-gain-approx}
%     % \quad or \quad \Bar{e} \approx \frac{a_{ego}}{k_f} 
% \end{equation}


% A smaller $I_{linear}$ is desirable as it corresponds to better SS. If $I_{linear} > 0$ the speed change is amplified from leader to the follower, yielding a string unstable case. 


% Remarkably, the our SS analysis here is also consistent with the theoretic analysis of SS in frequency domain, i.e. the larger time headway can reduce the $\infty-$norm and $2-$norm of the string stability transfer function in \cite{naus2010string, 5399965, gong2019cooperative}.



________________________________________________

% \subsection{PI in Laplace domain}

% \begin{align*}
%     u(t) &= k_p e(t) + k_i \int_{0}^{t} e(\tau) d\tau  \\
%     U(s) & = k_p E(s) +k_i \frac{E(s)}{s}
% \end{align*}


% \subsection{maybe ODE solution?}
% \section{Mathematical proof}\label{math}

% The impact mechanisms of low-level controllers in the aforementioned two factory ACCs are studied analytically here. This is thanks to the assumption of the $compute\_gb$ and $gb2accel$ functions, i.e. the desired acceleration requested by the $control$ will approximately equal to the true acceleration $a_{ego}$ responses from the car, which means:
% \begin{equation}
%     a_{ego} \approx control = k_p \cdot e + k_i \cdot \int_{0}^t {e(\tau)d\tau} +k_f \cdot a_{pid}
% \end{equation}

% \subsection{PI low-level controller and its impact on SS}
% First we investigate the impact of a PI controller given a linear upper planner.
% Consider that the proportional gain has a dominant effect, we omit the integral term for now which leads to:
% \begin{equation}
%      a_{ego} = control \approx k_p  (v_{pid}-v_{ego})
%      \label{P-dynamics}
% \end{equation}

% For a linear planner as \eqref{desire_d} and \eqref{ACC-\vt}, it satisfies:
% \begin{equation}
% \begin{aligned}
%     % a_{ego} & = \dot{v_{ego}}  \nonumber \\
%     \dot{s_{ego}} & = v_{\text{lead}} - v_{ego} = v_{rel} \\
%     \dot{s_{des}} &=  \tau \dot{v_{\text{lead}}} \\ 
%     \dot{v_{\text{lead}}} & = a_{\text{lead}}
%     \label{ACC}
% \end{aligned}
% \end{equation}
% Substitute \eqref{ACC} into \eqref{ACC-\vt}, we have: 
% \begin{equation}
%     \dot{\vt} = k (v_{\text{lead}}-v_{ego}) + (1-k  \tau) a_{\text{lead}}
%     \label{\vt_rate}
% \end{equation}

% To further investigate the impact on SS, we derive maximum changes in the ego vehicle target speed, namely $\Delta \vt$, which can be calculated by tracking \eqref{\vt_rate} from the time $T_1$ when the ego car starts to react to the lead vehicle to the time $T_1+\Delta T$ when the ego car stops from moving towards the lead vehicle's speed change and possibly starts to reduce the overshoot; see Fig.\ref{undershooting_actuator} (e). We have:
% \begin{align}
%     \Delta \vt & = \vt(T_1+\Delta T)- \vt(T_1) \nonumber \\
%     & = \sum_{T_1\le \hat{t} \le T_1+\Delta T} k (v_{\text{lead}}(\hat{t})-v_{ego}(\hat{t})) dt + (1-k  \tau) a_{\text{lead}}(\hat{t}) dt \nonumber \\
%     & =  (1-k  \tau) \overline{a}_{lead} \Delta T + k \sum_{T_1\le \hat{t} \le T_1+\Delta T} v_{rel}(\hat{t})
%     \label{analysis}
% \end{align}
% where $\overline{a}_{lead}$ is the average acceleration for the lead vehicle during $\Delta T$. Since $v_{\text{lead}}$ and $a_{\text{lead}}$ do not change with the follower, the magnitude of the speed change for the ego vehicle will only depend on $v_{rel}$. Also notice that $1-k \tau>0$ for rational values. Further, substituting $v_{ego} \approx \vt-e$ into \eqref{analysis}, we have:
% \begin{equation}
%     \Delta \vt = (1-k  \tau) \overline{a}_{lead} \Delta T + k \sum_{T_1\le \hat{t} \le T_1+\Delta T} v_{rel} ^{target} (\hat{t}) + k \sum_{T_1\le \hat{t} \le T_1+\Delta T} e(\hat{t})
% \end{equation}
% where $v_{rel} ^{target} (\hat{t}) = v_{\text{lead}}(\hat{t})-\vt(\hat{t})$.

% To evaluate the follower speed amplification magnitude we subtract the lead vehicle speed change $\Delta v_{\text{lead}}$ during $\Delta T$, which defines the index $I_{linear}$ for both acceleration or deceleration:
% \begin{align}
%   I_{linear} = & \frac{|\Delta \vt|-|\Delta v_{\text{lead}}|}{|\Delta v_{\text{lead}}|} \nonumber \\
%   & = k (\frac{\sum_{T_1\le \hat{t} \le T_1+\Delta T} |v_{rel}(\hat{t})|}{|\Delta v_{\text{lead}}|}- \tau) \nonumber \\
%   & \le k (\frac{\sum_{T_1\le \hat{t} \le T_1+\Delta T} |v_{rel} ^ {target} (\hat{t})| + |e(\hat{t})|} {|\Delta v_{\text{lead}}|}- \tau) \nonumber \\
%   & = k (\frac{|\Bar{v}_{rel} ^{target}| + |\Bar{e}| }{|\Bar{a}_{lead}|}-\tau)
%     \label{SS-index-ACC}
% \end{align}
% where $\Bar{v}_{rel}$ is the average relative speed during $\Delta T$, \Bar{e} is the average speed tracking error during $\Delta T$. A smaller $I_{linear}$ is desirable as it corresponds to better SS. If $I_{linear} > 0$ the speed change is amplified from leader to the follower, yielding a string unstable case. Correspondingly, we can notice the adversarial impact of a slow low-level controller, as it takes longer time for the speed tracking error $e$ to decay, which will induce larger value of $I_{linear}$, amplifying the speed fluctuations.

% %Although \eqref{SS-index-ACC} does not directly involve low-level variables, the impact of the mere low-level controller becomes straightforward. For a fixed planner, a slow-response controller moves the follower more slowly, which further makes the relative speed $v_{rel}$ larger, and also takes longer $\Delta T$ to stabilize. A faster controller can track the planned speed faster, reduces the speed amplification $\Delta \vt$ and thus improves SS. 

% The index in \eqref{SS-index-ACC} also sheds some light to the impact of the planner. Note that $k$, i.e., how fast the planner react to spacing, and the desired headway $\tau$ both affect SS as well. If the planner is more sensitive to spacing change (i.e., with a larger $k$), the ACC system is more likely to be string unstable (i.e., larger $\Delta \vt$ will make the planned trajectory harder to track). For the impact of $\tau$, \eqref{SS-index-ACC} indicates larger headway can benefit the SS, which is consistent with the recent empirical finding \citep{li2021ACC} from a few commercial ACC systems. 


% \textbf{In fact, the index can be viewed as the ratio, which is just the transfer function used in frequency domain. Here we keep it in time domain in order to introduce the impact from both of planner and low-level controller. }

% Remarkably, the our SS analysis here is also consistent with the theoretic analysis of SS in frequency domain, i.e. the larger time headway can reduce the $\infty-$norm and $2-$norm of the string stability transfer function in \cite{naus2010string, 5399965, gong2019cooperative}.

% \subsection{Proof of the SS for the linear planner}
% Although we adopted a new index to measure SS, it can be shown that the linear planner discussed in this paper in \eqref{ACC-\vt} is string stable, if $0 \le k \tau \le 2$.

% \begin{proof} We first convert the time-domain planner trajectory in \eqref{ACC-\vt} into frequency domain:
% \begin{equation}
%     \vt(j\omega) = k [x_{\text{lead}}(j\omega) - x_{ego}(j\omega) - \tau v_{\text{lead}}(j\omega)] + v_{\text{lead}}(j\omega)
%     \label{linear_freq}
% \end{equation}
% where $\omega$ is the angular frequency, $j$ is the complex number indicator. As here we focus merely on the planner, we assume $v_{ego}=\vt$. Then substituting in \eqref{desire_d}, and applying the position as the integrator of corresponding speed: $x_{\text{lead}}(j\omega) = v_{\text{lead}}(j\omega)/j\omega$, and $x_{ego}(j\omega) = v_{ego}(j\omega)/j\omega = \vt(j\omega)/j\omega$, we can rearrange \eqref{linear_freq} into the well-known speed to speed transfer function used in SS analysis \citep{}:
% \begin{equation}
%     \frac{\vt(j\omega)}{v_{\text{lead}}(j\omega)} = \frac{j(1-k \tau)\omega + k}{j\omega + k}
%     \label{\vt_freq}
% \end{equation}
% As $0 \le k \tau \le 2$ indicates $|1-k \tau| \le 1$, we can ensure that:
% \begin{equation}
%      \left \|\frac{\vt(j\omega)}{v_{\text{lead}}(j\omega)} \right\|^2 _2= \frac{[(1-k \tau)\omega]^2 + k ^2}{\omega^2 + k ^2} \le 1
%     \label{\vt_freq}
% \end{equation}
% which satisfies the frequency-domain SS criterion (\cite{naus2010string,Feng2019StringSF}): $\left \|\frac{\vt(j\omega)}{v_{\text{lead}}(j\omega)} \right\|_\infty \le 1$, indicating the string-stable property of the linear planner. Note that $\| v(j\omega) \|_\infty = \max _{\omega \in \mathbb{R}} v(j\omega)$, and $\| v(j\omega) \|_2 = \sqrt{\frac{1}{2\pi} \int_{-\infty}^{\infty} \text{Trace} [v(j\omega)^{\dagger}v(j\omega)] d\omega}$, $\dagger$ means the conjugate transpose.
% \end{proof}

% \subsection{PIF low-level controller and its impact on SS}

% As stated before, a PIF controller usually works with an MPC planner. Recall Algorithm 2 uses $a_{\text{target}}$, $v_{start}$ and $a_{start}$ to calculate the low-level setpoints $v_{pid}$ and $a_{pid}$. 

% In \eqref{a_{start}-v_{start}}, we can assume the initial $a_{start}$ equals to zero, thus the $a_{start}$ sequence can be simplified using only $a_{\text{target}}$ from the MPC planner, which leads to:

% \begin{equation}
% a_{start}(\hat{t}) = \sum_{n = 0} ^{\floor{\hat{t}/d\hat{t}}-1} \frac{d\hat{t}}{d t_{p}} (1-d\hat{t}/d t_{p})^{\floor{\hat{t}/d\hat{t}}-1-n} a_{\text{target}}(n d\hat{t})
% \label{vstart-iteration}
% \end{equation}
% where $\floor{\hat{t}/d\hat{t}}$ is a floor function to calculate index for planning step of $\hat{t}$ starting from zero. Substitute \eqref{vstart-iteration} into \eqref{a_{start}-v_{start}}, the changes of $v_{start}$ can be described using $a_{\text{target}}$ from the planner:

% \begin{equation}
% 2/d\hat{t} \cdot \Delta v_{start} = \sum_{T_1\le \hat{t} \le T_1+\Delta T} a_{\text{target}}(\hat{t}) + \sum_{n = 0} ^{\floor{\hat{t}/d\hat{t}}} \frac{d\hat{t}}{dt_{p}} (1-\frac{d\hat{t}}{dt_{p}})^{\floor{\hat{t}/d\hat{t}}-1-n} a_{\text{target}}(n d\hat{t})
% \label{SS-a_{\text{target}}}
% \end{equation}


% Correspondingly, the SS index $I_{mpc}$ given a MPC planner can be derived as:
% \begin{align}
%   I_{mpc}&= \frac{|\Delta v_{start}|-|\Delta v_{\text{lead}}|}{|\Delta v_{\text{lead}}|}\nonumber \\
%   &= -1 + \sum_{T_1\le \hat{t} \le T_1+\Delta T} |a_{\text{target}}(\hat{t})| \frac{d\hat{t}}{2|\Delta v_{\text{lead}}|} 
%     + \sum_{n = 0} ^{\floor{\hat{t}/d\hat{t}}} \frac{d\hat{t} (1-d\hat{t}/dt_p)^{\floor{\hat{t}/d\hat{t}}-1-n}}{dt_p|\Delta v_{\text{lead}}|}  |a_{\text{target}}(n d\hat{t})| 
%     \label{mpc-index}
% \end{align}

% Similarly, smaller $I_{mpc}$ means better SS.
% Here for an MPC controller, a slow low-level controller will trigger the planner to produce larger desired acceleration $|a_{\text{target}}(n d\hat{t})|$ and thus increase the  $I_{mpc}$, which means the SS is undermined. 

% Now we have derived two indexes to measure the SS for the linear+PI and the MPC+PIF ACC systems. The mathematical derivations in \eqref{SS-index-ACC} and \eqref{mpc-index} do not have explicit low-level variables yet, but they suggest the same finding that a fast controller (which enables faster decay of tracking error) can help the SS and vice versa. \eqref{SS-index-ACC} and \eqref{mpc-index} also indicate the SS is a result of the coupling effect from both the planner and the low-level controller. The interactions between could be more complicated, or even intractable for a non-linear MPC or deep neural network planner in the future. To derive a full analytical solution is out of the scope for this paper and further study is ongoing towards this direction. 

% % \textbf{Notice that the SS indexes we derived here are different than the $l_2$ or $l_{\infty}$ stability derived using control theory.} We argue that the indexes here lead some advantages: i) it does not require an equilibrium initial state; ii) it better implies the impact of lead speed change and iii) 
% \subsection{PI in Laplace domain}

% \begin{align*}
%     u(t) &= k_p e(t) + k_i \int_{0}^{t} e(\tau) d\tau  \\
%     U(s) & = k_p E(s) +k_i \frac{E(s)}{s}
% \end{align*}


____________________________________________ introduction


With the development of vehicle automation, adaptive cruise control (ACC) systems are now widely available on commercial vehicles around the world. From the perspective of traffic flow efficiency, ACC systems are expected to achieve string stability (SS) to ensure that small perturbations do not amplify upstream within a platoon of vehicles 
\citep{4282789, Feng2019StringSF}, i.e., speed fluctuations should be dampened rather than amplified by the followers \citep{naus2010string, zhou2005range}. In recent years, the SS of market ACC systems has drawn increasing attention from the traffic flow community. Unfortunately, the market ACC products can only be treated as "black boxes" due to the proprietary technology.  As a result, related studies in  the literature are mostly data-driven; i.e., researchers often collect the driving behavior data of market ACC vehicles and then directly examine the SS features (e.g., \citep{makridis2021openacc,li2021ACC} ) or indirectly study the features by calibrating a model (e.g., \citep{gunter2019model,gunter2020commercially,shi2021empirical}) .   %In the past three years, more and more researchers are collecting and researching on factory ACC using collected data \citep{gunter2019model,gunter2020commercially,makridis2021openacc,li2021ACC,shi2021empirical}. 
For example, \cite{gunter2020commercially} found that most market ACC systems are string unstable.  \cite{li2021ACC} has shown that factory ACCs can amplify or dampen an oscillation (and overshoot or undershoot after the oscillation), depending on the ACC headway setting, speed level, and leader trajectory. \cite{shi2021empirical} obtained similar findings that large headway setting produces better SS while small headway usually induces perturbations to grow. \cite{li2020trade} suggested such property of factory ACC indicates there exists a trade-off between SS, mobility and safety. These empirical findings of the "black boxes" have discovered valuable features of the factory ACC systems, which, however, lack an explanation from the root of ACC controller design and execution. 

% On recent car models, ACC functionality is originally provided by radar manufactures, e.g. Bosch, Continental, who sell small units to automakers. Those ACC units usually integrate a built-in ACC algorithm with the radar module. In detail, an upper-planner receives the updated information from the radar and plans for the optimal trajectory, then a low-level controller tries to execute the trajectory by sending low-level commands (gas/brake or acceleration) to the car control interface. While it is still unclear whether automakers have modified the built-in ACC algorithms from radar manufactures, recent empirical studies \citep{li2021FD} have shown that ACC systems from different car models   behave similarly, which could be partially explained by the same radar service under the hood. For a comprehensive list of the major car manufactures and their radar/ACC service providers, readers are referred to our recent review paper \citep{zhou2021review}. 


% To benefit the traffic efficiency, ACC systems are expected to achieve string stability (SS) to ensure that small perturbations do not amplify upstream within a platoon of vehicles 
% \citep{4282789, Feng2019StringSF}, i.e., speed fluctuations should be dampened rather than amplified by the followers \citep{5571043, zhou2005range}. In recent years, the SS of ACC systems has drawn increasing attention from the traffic flow community. Unfortunately, the market ACC products can only be treated as "black boxes" due to the proprietary technology. As a result, related studies in  the literature are mostly data-driven. In the past three years, more and more researchers are collecting and researching on factory ACC using collected data \citep{gunter2019model,gunter2020commercially,makridis2021openacc,li2021ACC,shi2021empirical}. Notably, some interesting empirical features are reported. \cite{gunter2020commercially} found that most market ACC systems are string unstable. In contrast, \cite{li2021ACC} revealed factory ACCs can amplify or dampen an oscillation (and overshoot or undershoot after the oscillation), which is found appreciably depending on the ACC headway setting, speed level, and leader trajectory. \cite{shi2021empirical} obtained similar findings that large headway setting produces better SS while small headway usually induces perturbations to grow. \cite{li2020trade} suggested such property of factory ACC indicates there exists a trade-off between SS, mobility and safety. These empirical findings of the "black boxes" have discovered some important features of the factory ACC systems, which also requires better explanation. 
% An ideal conjecture of the factory ACC algorithms should be able to explain them.

% The recently empirical data have also inspired new modeling studies to approximate the ACC "black-boxes". 
% % But the analysis and formal methods in those new studies are still based on old-school theory.
% An optimal velocity relative velocity (OVRV) model was proposed in \cite{wilson2011car} for linear SS analysis of the ACC algorithms. \cite{gunter2019model} applied the same model to fit some field data of recent ACC-equipped cars, and found that the model is string unstable by simulations. Two more recent studies \citep{li2020trade,shi2021empirical} used a similar parsimonious linear CF model in which the follower acceleration is only proportional to spacing change. They found that the model falls short in explaining some empirical ACC features, and conjectured that in practice the control sensitivity factor of factory ACC are unlikely to be a constant. These studies on modeling of factory ACCs suggest that, linear CF models in literature might not be desired candidates for describing these "black boxes". More comprehensive alternatives are required. 

Although the data-driven studies have shed new light on understanding the factory ACC systems, there are some limitations.  Notably, in recent car models, ACC functionality is often provided by radar manufacturers, e.g. Bosch, Continental, who sell the units to automakers. Those ACC units usually integrate a built-in ACC algorithm with the radar module.  More specifically, an upper-planner receives the updated information from the radar and plans for the optimal trajectory, and then a low-level controller executes the trajectory by sending low-level commands (gas/brake or acceleration) to the car control interface.  %The recent empirical studies \citep{li2021FD} have shown that ACC systems from different car models behave similarly, which is probably because the ACC units were provided by the same radar manufacturer.  For a comprehensive list of the major car manufactures and their radar/ACC service providers, readers are referred to our recent review paper \citep{zhou2021review}.  
Given this design feature of ACC,  the data-driven approach is not ideal in uncovering ACC behaviors.  First, they use similar GPS devices with a sampling rate of only 0.1s, which  is larger than the typical updating interval for both radar (0.05s) and the low-level control system (0.01s) in modern cars. This means that some vehicle maneuver information is potentially lost.  Second, the data-drive approach only captures the holistic outcomes of ACC behaviors and cannot decouple the role of the upper-level planner and lower-level controller as well as their interactions.  Notably, the prevailing approach of model calibration per %All current studies to design string stable ACC systems 
\citep{gunter2019model,li2020trade,shi2021empirical} essentially captures only the upper-level planner and assumes that the low-level controllers achieve perfect performance as desired, which is questionable in real-world driving scenarios.  In fact, \citep{li2020trade,shi2021empirical} calibrated the factory ACC using a parsimonious linear CF model % in which the follower acceleration is only proportional to spacing change. 
and found that the model falls short in explaining some empirical ACC features.  This highlights the needs of going deeper into the mechanic level of ACC controller design and execution. 



%Second, the speed and distance measurements from GPS might be inconsistent with what a radar detects, as radars are known to be less accurate when the leading vehicle is far away or not moving. And many modern ACC modules integrate camera estimation for sensor fusion using specific state estimation algorithms.  %In addition, GPS measurement errors \citep{li2021FD} will increase the discrepancy with what a factory ACC really perceives. 


% Under this circumstance, the current approach to study SS of the factory ACC systems are far from perfect, mainly due to the missing of a prototype to describe the factory ACC structure. We anticipate a complete factory ACC model that can help better conjecture other market ACC products, explain those empirical findings and facilitate better SS design. It would also be desirable if not necessary for us to access the direct input (radar, camera) and output (low-level commands) of a ACC system, and even obtain the capability to modify and test the ACC algorithms. However, the car manufactures will most likely keep their ACC products proprietary due to patent privacy and technology-related protection, which stay against the expectation of academic researchers.

Fortunately, a recently open-sourced factory ACC system, Openpilot \citep{Openpilot}, here provides a feasible solution to overcome the proprietary issue.  %comes to "save the day". %provides us with a flexible and easily-accessible platform to research on factory ACC system%.
Openpilot is developed by an after-market self-driving company, Comma.ai. %, who aims to be to Tesla what Android is to Apple. 
Besides the open-source ACC software, Comma.ai also develops an after-market ACC development kit, Comma Two, which can connect the stock ACC unit and override its control on many regular commercial cars. Note that Openpilot is considered to be factory level because it only overwrites the built-in algorithms in the ACC unit, as it still uses the stock sensor and communicates with existing car control interface. The benefits of such open-source ACC software and after-market hardware are unprecedented. Openpilot enables researchers to obtain full access to all the controller parameters, variables and algorithms of the ACC system. It opens a new gate for analysis, design and test of our own factory ACC algorithms, which is aligned with the objective of this study.

Prior to the open-source factory ACC algorithms, the SS of ACC systems has already been extensively studied in the control area \citep{yanakiev,liang1999optimal,Liang2000StringSA}. 
The theoretical SS condition for linear CF models have been examined for years since \citep{wilson2011car}, and one can notice that it is not difficult to meet the SS condition after tuning the model parameters. For example, \cite{gunter2019model} obtained a wide region of string-stable parameters for the optimal speed velocity speed model and verified the SS through simulation.  \citep{wilson2011car} has derived the parameter domain for string stability for some of the models.  
%Besides the numerical studies, there are also a few real-car validations of string stable ACC planners or cooperative adaptive cruise control (CACC) algorithms \citep{naus2010string,6082981,milanes2013cooperative,Lu2018TruckCS,Eilbert2020PerformanceCO}. 
Yet, some interesting questions arise: why string-stable commercial ACCs are very rare in real life? Can we directly apply those tuned models to a car and achieve string-stable performance? %, while the SS condition of the ACC planners are easy to satisfy? For those car experiments in literature, can they be easily generalized to daily car models?  
Unfortunately, the current short answers are "no". This study specifically points out that the gap between SS theory and practice lies in the impact of low-level controller, which has been consistently neglected so far. 
% We argue that, any design of ACC planners without a low-level controller is incomplete, since how well the planned trajectory can be executed will remain unknown. 
For the field experiments in literature, researchers used either original equipment manufacturer (OEM) controller or in-house designed controllers. The OEM controller \citep{Eilbert2020PerformanceCO} directly tracks the acceleration/speed command, or torque/brake pressure generated from the upper-level planner but the algorithms are also 'black-boxes'. The in-house designed controllers use specific feedback control law to track the planning trajectories, e.g. \cite{naus2010string,6082981} used a MOVE gateway to interact with the vehicle motor to achieve acceleration setpoint ; \cite{Lu2018TruckCS} applied feedback linearization control to calculate the desired torque/brake pressure command of truck actuators for desired accelerations; and \cite{Shladover2009EffectsOC} utilized the loop-shaping techniques to devise a speed servo to track the planned speed. Although the in-house designed controllers demonstrate desired performance in the experiments, they are only applied to specific filed-test scenarios, it's unclear if they can be generalized to real-world driving. Additionally, most in-house designed controllers are not open-sourced either. 


Correspondingly, with an emphasis on analyzing the impact of the factory low-level controller, this study first presents the open-source factory ACC algorithms, based on which we further investigate the impact of low-level controller on SS. The findings will be validated through both numerical simulations and real-car tests on a regular commercial car model, a 2019 Honda Civic.      

%66 for Danjue
The contribution of this paper is two-fold: i) for the first time we have introduced an open-source factory ACC system to the literature, which allows us to develop a new experimental method to test new ACC algorithms. The method can be easily implemented on most car models available on the market. Such a method provides promising opportunities to understand the market "black boxes". ii) We have shown that the impact of low-level controller on string stability is significant, which has been neglected in the literature. This finding suggests a new direction to tackle the SS issue in controller design.

The remainder of the paper is organized as follows: section II introduces the factory ACC algorithms for both planner and low-level controller; section III investigates the impact mechanisms of the low-level controller on SS; section IV presents the experimental method; section IV showcases the results and findings; section V concludes the paper and discusses future directions.




-----------------------------------
The paper has formulated the control algorithms in an open-source factory ACC system. We find that the factory ACC system, either the linear ACC or MPC, avoids to incorporate the low-level responses (e.g. ego vehicle speed or acceleration) in the planning loop. Such design might be due to some hardware consideration, but it clearly distinguishes the factory planners from a regular CF model or rule-based controller in the current literature. We point out the differences here and encourage further studies to investigate the impact of these changes on safety or traffic mobility. On the other hand, we find the factory ACC planner design is somewhat 'manual', still lacks the base theory and needs more improvement, especially for the MPC with more flexible cost objectives. For example, the desired distance of the MPC in \eqref{mpc-desireD} is quite different from that in the linear ACC \eqref{desire_d}. The purpose of this design is not straightforward and definitely needs more justifications. The weights for different sub-costs in \eqref{MPC-cost} are often empirically chosen which also needs more theory regarding the safety or SS performance. Future studies are encouraged to work towards this direction. The other type of upper-level planners, such as the CF models or end-to-end vision-based longitudinal controllers, are also highly recommended. Along this, we have already implemented the IDM model in the shared repository, whose results will be included in our sequel paper.

The study focuses on the impact of the low-level controller on SS. Through analysis of impact mechanisms we find a slow low-level controller can undermine SS despite a string-stable upper-level planner. Besides, the integral term in the low-level controller also causes overshooting that affects SS. Numerical and real-car experiments further demonstrate that a slow low-level controller can result from either the insufficient P/F gains, or a weak gas/brake system, or both. A slow controller also amplifies the integral overshooting by accumulating greater tracking error. Accordingly, we suggest tuning up the proportional/feedforward gain and ensuring the gas/brake is strong enough. %not weak. 
Of course, the controller cannot be too fast to cause oscillations. For future studies, we suggest more investigation on the low-level controller to eliminate or reduce the downgrade of SS. 
%itno the novel design of the low-level controllers to help reduce tracking error, which could outperform the baseline PI/PIF controllers introduced here. 
Also, for considerations of the SS, in-depth analysis of the non-overshooting controllers is needed.  

The results and findings of this paper are based on the factory ACC algorithms in Openpilot, Comma.ai. While the stock ACC algorithms on commercial car models vary and remain proprietary, we conjecture they %could 
follow a similar two-level control framework we introduce in this study, as they share the same ACC units from limited radar manufacturers. The factory ACC algorithms presented here help explain some recent empirical findings, such as the varying SS at different speed levels/ headway settings, the observed overshooting/undershooting at the end of an oscillation, and the puzzling gap between many string stable planner designs and string unstable platoons in real world. We believe the theory and methods in this paper provide a new and promising way for future studies to explain more empirical ACC features or approximate those "block-box" ACC products on the market. 


------------------------------

% and implements its algorithms in numerical simulations and on real car models.
% This study emphasizes on investigating how will a low-level controller impact the SS performance. 
% Through numerical and empirical experiments, we find that given a string stable upper-level planner, a fast-response low-level controller can improve SS, while a slow-response controller can undermine it. Moreover, the low-level controller cannot be too fast which will overreact and induce undesired oscillations. 
% Numerical and real-car experiments further demonstrate the a slow low-level controller can result from either insufficient P/F gains, or undershooting gas/brake system, or both. Besides, integral term can cause additional overshooting which worsens the SS. A slow controller amplifies the integral overshooting by accumulating greater tracking error.

% can be used as prototypes to explain the empirical features in ACC data or approximate the "block-box" ACC models. 

% We suggest future studies work on: i) novel designs of low-level controllers rather than the baseline PI or PIF controllers. Non-overshooting controllers are expected to improve SS.; ii) the trade-off between a faster low-level controller and driving comfortableness, safety, and traffic efficiency ;iii) other type of upper-level planners, such as the CF models or end-to-end vision-based longitudinal controllers. Along this, we have already implemented the IDM model in the shared repository, whose results will be included in our sequel paper. 


% This study opens the gate for the following directions:

% (i) We infer that it would be beneficial to pay more attention on improving the low-level controller rather than designing more string stable ACC models which have been extensively studied. We also anticipate better tracking performance of low-level controllers, compared to the baseline PI or PIF discussed here. We found that integral accumulation can affect SS and could potentially cause integral windup for slow controller. For anti-windup design, we believe the derivative gain can be leveraged to prevent integral windup and alleviate the overshooting issue. However, this will require further investigations and parameter tuninngs, since currently derivative is typically set to zero to avoid amplifying the measurement noises in accelerations.

% (ii) Regarding to the planner design, so far only the linear and MPC planners are widely investigated and applied, and no learning-based longitudinal planner has been officially reported on commercial vehicles yet \citep{zhou2021review}. Considering the learning-based controller is a trend for future autonomous driving, thereby, we would suggest researchers to leverage Openpilot to explore string-stable learning-based longitudinal planner. We also strongly recommend researchers from the traffic flow community to test different CF models as the new planners and investigate if CF models can outperform the linear/MPC controllers inherited from control domain. The authors have extended Openpilot to make it more friendly for testing CF models, and along this we have already tested IDM model, whose results will be included in our sequel paper.

% (iii) The impacts of road grade, curvature, and acceleration bound (due to vehicle actuator or comfort-related constraints) are not discussed in this paper. These factors require more attentions and investigation in both upper-level planner and low-level controller, such that SS can be fully realized in the real-world driving.


% The paper detailed the factory ACC algorithms and open-sourced a traffic-friendly package that allows testing of CF models. 

% Some limitations and discussion on future studies are listed below:
% \begin{enumerate}[label=\Roman*]
%     \item Although we suggest tuning a fast low-level controller, this paper does not quantify how fast the controller needs to be to guarantee the SS given a certain planner. Notice that a too fast controller certainly causes oscillations in real life which sabotages driving comfortableness. Therefore we need careful tuning on real cars to seek some balance point experimentally. We managed to achieve this for MPC+PIF easily, which feels safe and comfortable. But linear+PI seemed more tricky and a fast low-level controller gave us jerky experiences. The differences between the two systems are worth further investigation. Unfortunately the mathematical derivations in \ref{math} still expresses SS as a result of both the planner and the low-level controller. This is mainly due to the complex interactions between the planner and low-level controller. While we are not sure they are mathematically tractable, we believe more analysis can be done along this, and more specific instructions on tuning the low-level controller could be provided with respect to different planner designs. 
%     \item Methods introduced in this paper are expected to benefit future studies. We strongly recommend readers from the traffic flow community to test different CF models as the new planners and try to outperform the linear/MPC controllers inherited from control domain. The authors have extended Openpilot to make it more friendly for testing CF models, and along this we have already tested IDM model, whose results will be included in our sequel paper.  
%     \item We have derived a more general indexes to measure the SS, extending the traditional definition that requires strict equilibrium state as the initial condition. We argue that the two indexes for linear and MPC controller; see \eqref{SS-index-ACC} and \eqref{mpc-index}; are better than norm-based SS condition in the following aspects: i) ; ii) and iii) 
%     \item The results and findings of this paper were derived based on the factory ACC algorithms in Openpilot. While the stock ACC algorithms on different car models are varied and remain proprietary, we conjecture that they will mostly likely follow a similar framework as we introduced here, because they are using same radar modules that has built-in ACC functionality. Speaking of the planner design, so far only the linear and MPC planners are widely studied and applied, and no machine learning longitudinal controller has been officially reported yet \citep{zhou2019longitudinal}. Thus it is safe to say the two streams of ACC algorithms introduced here can serve as baselines. We also believe they can be used as surrogate models to investigate those "black-box" ACC modules on commercial vehicles. Towards this, it is suggested to leverage the open-source factory ACC algorithms to explain the ACC features observed from empirical data. For example, the impact of headway on SS, can be well explained using some of the factory models in \eqref{SS-index-ACC}. Also, we can use those ACC models to fit the empirical data with necessary modifications. 

%     \item We also expect better low-level controller design than the baseline PI or PIF discussed here. Derivative is typically set to zero to avoid amplifying the noises in accelerations. We also found that integral windup undermines SS. For anti-windup design, we believe the derivative gain can be leveraged to prevent integral windup and alleviate the overshooting issue. 
% \end{enumerate}





% The findings of this paper implies the SS might not be achieved in all circumstances. The paper finds a slow low-level controller undermines SS, which is almost inevitable in real life. Even if desired control gains are pre-tuned by ACC manufactures, the gas/brake on cars might degrade the over time, cause undershooting and leads to a slow low-level controller. A slow low-level controller could also result from grades, or heavy loads, which are not accounted by constant low-level controller design. 

% Except the findings on the impact of low-level controller, this work, for the first time, detailed the two types of factory ACC algorithms open-sourced by Openpilot, i.e. a linear+PI and an MPC+PIF.









% The procedure is to gradually increase the P gain and the evaluation principle is to balance the tracking performance and the disturbance rejection, because faster tracking contradicts to  which is a common trade-off for nearly all PI/PIF controllers. For more advanced methods in balancing the fundamental two goals and improve the stability of the controller, there exists a plethora of studies \citep{nie2020energy} tackling it as an optimization problem. Many instructions and tools are also available online \citep{balance}.  

% Based on this, one can tune the control gains for faster tracking while not causing large disturbances. 

% More advanced tuning methods have also been developed by formulating it as an optimization problem, whose objective is to improve the tracking performance, the robustness, 
% but to the best of our knowledge, there does not exist a general method to get the 

% Starting from the initial values, we can keep increasing/decreasing until the oscillations are observed. 

% For instance, the default $P$ gain of the PI controller in Openpilot is $k_p(v) = 1.2 - 0.02 v$ for $v \in [0,35]$.

% However, in practice, a fast-response controller might cause other impacts, e.g. less driving comfort, more emissions or even instability. Such effects vary on differently car models due to different sensitivities of powertrain, suspensions and the road conditions. Therefore, there does not exist any explicit unique control gains applicable to all cars. The general principle suggested by this paper is to tune up the control gain while it still remains within a proper range constrained by other essential needs, including controller stability and driving comfort.
% Based on the argument aforementioned, we now provide some feasible procedures on the experimental design of low-level controller. 
% We first conduct a stability analysis to determine the proper range of gains. A first point of analysis is whether the system converges or diverges. A second point of analysis is whether the system exhibits oscillatory or smooth behavior.
% Of course, the controller cannot be too fast to cause oscillations. For future studies, we suggest more investigation on the low-level controller to eliminate or reduce the downgrade of SS. 
% Also, for considerations of the SS, in-depth analysis of the non-overshooting controllers is needed.  



------------------

Recalling the pipeline in Fig.\ref{pipeline}, a low-level controller is tunable in terms of both the control gains and the $compute\_gb$ function in pair with the gas/brake system, aka $gb2accel$ function. To design a fast low-level controller, first we need to ensure the gas/brake is not weak. For this we suggest collecting some real driving data of a specific car model and fit the relationship between gas/brake and accelerations, as shown in Fig.\ref{accel2gb_relation}. It would help us approximate the $gb2accel$ function based on which we can design the corresponding $compute\_gb$ function to ensure the actuator produces enough gas/brake that $control$ requests. Then we focus on tuning the control gains. For a regular PID controller, a heuristic method to obtain the control gains was first proposed by \cite{Ziegler1942OptimumSF}, which works as follows:
(i) setting the integral gain and derivative gain to zero;
(ii) gradually increasing the proportional gain until the closed-loop system exhibits oscillatory behavior. Then record the corresponding proportional gain as $k_{\text{cr}}$, and the oscillation period as $P_{\text{cr}}$;
(iii) determine the values of the control gains using $k_{\text{cr}}$, $P_{\text{cr}}$ by referring a table \citep{ZNmethod}.
% \begin{table}[ht]
% \caption{Recommended control gains by Ziegler-Nichols method for a regular PID controller}
% \centering
% \begin{tabular}{ |c|c|c|c| } 
%  \hline
%  Controller type & $k_p$ & $k_i$ & $k_d$ \\ 
%  \hline
%  P & $0.5 k_{\text{cr}}$ & 0 & 0 \\ 
%  \hline
%  PI & $0.45 k_{\text{cr}}$ & $1.2 k_p/P_{\text{cr}}$ & 0\\ 
%  \hline
%  PID & $0.6 k_{\text{cr}}$ & $2 k_p / P_{\text{cr}}$ & $0.125 P_{\text{cr}} k_p$\\ 
%  \hline
% \end{tabular}
% \end{table}
The classical Ziegler-Nichols method can provide the initial workable values for a regular PID controller with constant gains, but here for a speed tracking controller, we need more complex design because the gains have to work under a wide spectrum of speed levels, ranging from 0 m/s to 35 or 40m/s,  where the accelerating/decelerating capabilities change significantly. This causes more challenges for determining the control gains. An engineering solution could be repeating the Ziegler-Nichols method at a few speed levels and interpolating gain values between points. But it's unclear which speed levels should be used.

Here we suggest incorporating the linear acceleration model \citep{rakha2001vehicle,laval2014parsimonious,xu2020statistical} in traffic flow domain to derive the initial control gains. In the model, the desired acceleration of a free-motion vehicle is found linearly dependent on speed, i.e. $a(v) = a_{0}(1-v/v_{max})-gG$, where $g$ is the gravity acceleration, $G$ is the grade, $a_{0}$ is the maximum acceleration and $v_{max}$ is the maximum desired speed. Such linear acceleration model for human drivers also suggests the shape of acceleration bounds for a self-driving car; see the default values used by Openpilot in Fig.\ref{accelboundandgains}. 
Recall that the $control$ variable from the low-level controller in \eqref{PI_eq} is an approximation of the true acceleration $a_{ego}$. The maximum true acceleration induced by the low-level controller should be close to the acceleration bounds adopted by human drivers for satisfying driving comfort. Then we have:
\begin{align}
    % \max_{t} a_{ego}(v)  &= a(v) \\
%   &\max \{ gb2accel(compute\_gb(control)) \} \leq a_{max}^d (v)\\
     k_p(v) \cdot e_{max} &\approx a(v) 
    %  k_p(v) &\approx  a(v)/e_{max}
\end{align}
where $e_{max}$ is the maximum speed error in the low-level control loop. From Algorithm 1, one can see $e_{max} = oa=2 m/s$, thus the initial P gain $k_p \approx a(v)/e_{max} = a(v)/2$. 
To compute the initial values for the I gains, a common method is to first determine how long it will take for an integral action to match a proportional action. For example, if the ideal time is 10 steps in the control loop, then it leads to $\Sigma_{1}^{10} k_i(v) e \approx k_p(v) e$, i.e. $k_i(v) \approx k_p(v)/10$. 
Starting from those initial values, one needs to first tune the controller to meet some essential requirements for a self-driving car, such as increasing the gains at low speeds for quick start-up, or making the controller more responsive at high speeds for safety concerns. This procedure requires lots of engineering experience from empirical testing. We show an example of the default control gains used in Openpilot; see Fig.\ref{accelboundandgains}. Those values may satisfy the basic driving needs but not necessarily benefit the SS of our interests. 
% Notice that the relationship between acceleration bounds and final P gains are altered due to default values used in Openpilot; see Fig.\ref{accelboundandgains}.   
\begin{figure}
    \centering
    \includegraphics[width=0.5 \textwidth]{controlgain.png}
    \caption{Acceleration bounds and the default PI control gains in Openpilot (for a 2019 Honda Civic)}
    \label{accelboundandgains}
\end{figure}
% \FloatBarrier
The next step is to tune fast the controller to facilitate the SS. To achieve this, we suggest to remain the shape of function $k_p(v)$ and add a scaling factor for further tuning, i.e. $s \cdot k_p(v)$ where $s$ should be gradually increased from 1. For tuning the controller to get high response dynamics, there are many instructions, handbooks and tools, e.g. \citep{handbook,tunefast} available online. More advanced tuning methods can also be found in literature \citep{wang2000optimal,o2006pi,kanojiya2012optimal}. The general procedure is to gradually increase the gains while not causing instability. It can be done by guess and check method as well. To check new control gains, one can evaluate the SS performance by running platoon experiments in simulations as shown in Fig.\ref{P-gain}, as it is cheap and safe to do. We keep increasing the low-level control gains until the desired SS is achieved in simulations. Then the real car experiments are recommended for further testing because some other aspects such as the driving comfort, the impact of grades, or sudden disturbances also need to be accounted. The SS can also be verified by real car experiments as Fig.\ref{real-fast-slow} shows.


The paper has formulated the control algorithms in an open-source factory ACC system. We find that the factory ACC system, either the linear ACC or MPC, avoids to incorporate the low-level responses (e.g. ego vehicle speed or acceleration) in the planning loop. Such design might be due to some hardware consideration, but it clearly distinguishes the factory planners from a regular CF model or rule-based controller in the current literature. We point out the differences here and encourage further studies to investigate the impact of these changes on safety or traffic mobility. On the other hand, we find the factory ACC planner design is somewhat 'manual', still lacks the base theory and needs more improvement, especially for the MPC with more flexible cost objectives. For example, the desired distance of the MPC in \eqref{mpc-desireD} is quite different from that in the linear ACC \eqref{desire_d}. The purpose of this design is not straightforward and definitely needs more justifications. The weights for different sub-costs in \eqref{MPC-cost} are often empirically chosen which also needs more theory regarding the safety or SS performance. Future studies are encouraged to work towards this direction. The other type of upper-level planners, such as the CF models or end-to-end vision-based longitudinal controllers, are also highly recommended. Along this, we have already implemented the IDM model in the shared repository, whose results will be included in our sequel paper. 



The results and findings of this paper are based on the factory ACC algorithms in Openpilot, Comma.ai. While the stock ACC algorithms on commercial car models vary and remain proprietary, we conjecture they follow a similar two-level control framework we introduce in this study, as they share the same ACC units from limited radar manufacturers. The factory ACC algorithms presented here help explain some recent empirical findings, such as the varying SS at different speed levels/ headway settings, the observed overshooting/undershooting at the end of an oscillation, and the puzzling gap between many string stable planner designs and string unstable platoons in real world. We believe the theory and methods in this paper provide a new and promising way for future studies to explain more empirical ACC features or approximate those "block-box" ACC products on the market. 

Current market ACCs are only level-2 self-driving systems which are rule-based, and the industry is moving towards the level-5 system using machine learning methods based on neural networks. It's likely that the SS achieved on rule-based level-2 ACCs will be sacrificed in the future due to totally different models. While one can derive mathematically the SS condition for a rule-based linear planner, to guarantee the SS in machine learning ACC models certainly needs more investigation. An ongoing study from the authors is aimed at this goal to train string stable machine learning ACCs for future cars.  














---------------------------------------------------

The discussion we had before Peeta's edits;


\section{Discussion and Outlook}
% the classical way to derive control gains for PID
% recent optimization methods to improve PID (what are the measures they are using?)
% a fast controller means better tracking performance
% tune up the control gain while not against the stability
% for speed controller, it has to be speed dependent
% the tuning of PID is to balance reference tracking and disturbance rejection. Methods and tools have been developed towards this goal. 
The study has investigated the impact of the low-level controllers on the SS which has been ignored so far.
The major finding is that a fast-tracking low-level controller is essential to ensure the SS even if the upper-planner is string stable. 
%Accordingly, we include the following discussions on tuning fast low-level controllers to achieve SS on factory ACC products.
%As the recent aftermarket tools such as Comma Two and Openpilot enable more and more users to modify and customize the ACC systems for their own vehicles, we conjecture the customization trend on personal cars will keep growing and strongly recommend users to tune their low-level controllers for fast tracking performance in order to benefit the traffic while not causing safety hazards. To assist this, now we provide some practical guidance on how to tune a fast low-level controller. 
In order to improve the SS and benefit the traffic flow, we provide the following practical guidance on how to tune a fast low-level controller. 

\subsection{Guidance on tuning the low-level controllers}

The Ziegler-Nichols method \citep{Ziegler1942OptimumSF} is commonly used to obtain the control gains for a PID controller, whose procedure is basically to first set the integral and derivative gain to zero and gradually increase the P gain until the system exhibits oscillatory behavior. Then, a look-up table procedure gives the estimated values of control gains. 


In this study, we propose an extension of the Ziegler-Nichols method (which only considers constant control gains), since our control gains $k_p(v)$ are speed-dependent. We propose the following two-step method: the first step is to obtain the an initial feasible $k_p(v)$, in that it should be able to track the speed reference and drive the car. The second step is to fine tune $k_p(v)$ to achieve a fast low-level controller for better SS. 

% To tune the control gains for a fast low-level controller, we first need to obtain the initial workable values. 
% A common method for computing the control gains of a PID controller was proposed by \cite{Ziegler1942OptimumSF}, where


%The Ziegler-Nichols method can provide the initial workable values for a regular constant-gain controller, but here for a speed tracking low-level controller, we need more complex design because it needs to work under a wide spectrum of speed levels, where the accelerating/decelerating capabilities change significantly.
% This complexity causes more challenges for determining the control gains. An engineering solution could be repeating the Ziegler-Nichols method at a few speed levels and then interpolating, but it is unclear what speed levels should be used.

To derive the initial P gains of the low-level controller  we conjecture that they should be proportional to the maximum acceleration the engine is able to output, namely  $a^*(v)$.   \cite{rakha2001vehicle} has shown that a straight line provides a good fit to this function. Notice that a straight line fit also matches empirical data of the desired acceleration of human driven vehicles \citep{laval2014parsimonious,xu2020statistical}.
Since $a^*(v)$ is the upper bound for the acceleration, it should satisfy:
\begin{align}
    a^*(v) &\geq \max a_{ego}(v) 
\end{align}

To see why our conjecture should be robust, combine \eqref{sim-dynamics} and \eqref{controlequal} to get:
\begin{equation}
     k_p(v) \cdot e(t) \approx a_{ego}(v(t))
    \label{controlequalaego}
\end{equation}
And from Algorithm 1 we see the maximum speed error in the low-level controller is $\max e(t)=2m/s$. Thus the maximum acceleration generated by the low-level controller is $\max\limits_{t} a_{ego}(v) \approx 2k_p(v)$ at speed $v$, which indicates the P gain $k_p(v)$ is a multiple of the maximum acceleration. 

The maximum acceleration in control design should be approximately equal to the true acceleration bound limited by the engine, which gives:
\begin{align}
    k_p(v) & \le a^*(v)/2
    \label{multiple}
\end{align}

The default acceleration upper bound used in Openpilot can be seen in Fig.\ref{initialP} (a), which is piece-wisely linear and larger than the human drivers’ linear accelerations. If we assume $a^*(v) = 1.0(1-v/40)+0.5$ for a regular car model, then use \eqref{multiple} we can derive the initial P gains $k_p(v) =0.5(1-v/40)+0.25$. We test the performances of such initial P gains in simulations; see Fig \ref{initialP} (b); which are feasible for driving but string unstable. The results validate our approach to derive the initial P gains. 
For the initial values of the I gains, a common method is to first determine how long it will take for an integral action to match a proportional action. For example, if the ideal time is 10 steps in the control loop, then it leads to $\Sigma_{1}^{10} k_i(v) e \approx k_p(v) e$, i.e. $k_i(v) \approx k_p(v)/10$. 



\begin{figure}[!htbp]
\centering
\begin{subfigure}[t]{0.45\linewidth}
    \includegraphics[width=\linewidth]{initialP.png}
    \caption{Default acceleration bound and control gains in Openpilot}
\end{subfigure}%
\begin{subfigure}[t]{0.45\linewidth}
    \includegraphics[width=\linewidth]{initialP_SS.png}
    \caption{Performance of the initial gains from linear acceleration model}
\end{subfigure}%
    \caption{Default P and I gains in Openpilot and the initial P gain using linear acceleration model: $k_p$ and $k_i$ are the default control gains, $a(v)$ is the linear acceleration bound, and $a(v)/2$ is the proposed initial P gain }
    \label{initialP}
\end{figure}
\FloatBarrier

% Starting from those initial workable gains, the next step is fine-tuning. First, we need to tune the gains to meet the essential driving requirements, such as increasing the gains at low speeds for quick start-up, and making the controller more responsive at high speeds for safety concerns. This procedure requires lots of engineering experience. We show an example of the default control gains used in Openpilot; see Fig.\ref{initialP} (a). Those values have been tuned by engineers which meet the basic driving needs but not necessarily guarantee the SS . 

Next we tune the control gains for the fast tracking performance. To this end, we suggest keeping the shape of $k_p(v)$ and only tuning a scaling factor before it, i.e. $s \cdot k_p(v)$ where $s$ should be gradually increased from 1. For tuning the controller faster, there exists many instructions, handbooks and tools, e.g. \citep{handbook,tunefast} online. More advanced tuning methods can also be found in literature \citep{wang2000optimal,o2006pi,kanojiya2012optimal}. The general procedure is to gradually increase the gains while not causing instability. The most straightforward method is trial-and-error. To check the new control gains, one can evaluate the SS performance by running the platoon experiments in simulations as shown in Fig.\ref{P-gain}, as it is efficient and hazard-free. We keep increasing the control gains until the desired SS is achieved in simulations. Then the real car experiments are recommended for further testing because some other aspects such as the driving comfort, the impact of grades, or sudden disturbances also need to be accounted. The SS can be evaluated from the experiments as shown in Fig.\ref{real-fast-slow}. 

The proposed procedures are designed for a PI controller. The initial control gains for the PIF low-level controller are easier to find, for example $k_f=1.0$, $k_p=0.0$ and $k_i=0.0$. We can tune fast the controller following a similar procedure discussed above.

To ensure the gas/brake is strong enough, we suggest collecting some real driving data of a specific car model; see Fig.\ref{accel2gb_relation}; and fit the actuator model in \eqref{gb2accel}, based on which we can design the $compute\_gb$ function to ensure the actuator is strong. 

\subsection{Future research}

The results and findings of this paper are based on the open-source factory ACC algorithms in Openpilot, Comma.ai. While the stock ACC algorithms on the commercial car models may vary and still remain proprietary, we conjecture they follow a similar two-level control framework introduced in this study, as they share the same ACC units from limited radar manufacturers. To provide more evidence, the factory ACC algorithms presented here are able to explain some recent empirical findings from factory ACC vehicles, such as the varying SS at different speed levels/ headway settings, the observed overshooting/undershooting at the end of an oscillation, and the puzzling gap between many string stable planner designs and string unstable platoons in real world. 
We believe the theory and experimental methods in this paper provide a new and promising way for future studies to explain more empirical ACC features or approximate those "block-box" ACC products on the market. 


To encourage more experimental testing of ACC algorithms on real cars, the authors have shared a custom fork of Openpilot  \footnote{\url{https://github.com/HaoZhouGT/openpilot}}. This repository includes the implementation of the linear ACC+PI and MPC+PIF frameworks presented in this paper. The low-level controllers are fine-tuned for a 2019 Honda Civic and interested readers are welcome to test them in the filed. We have added a parser to process the raw log files from Comma Two and help retrieve the ACC variables and the CAN bus signals.  
It is worth noting that the experimental method not only applies to the study of the low-level controllers. Any design of the ACC algorithms, e.g. a new planner model, can be tested in the same way. 


The paper has formulated the control algorithms in an open-source factory ACC system. We find that the factory ACC system, either the linear ACC or MPC, avoids to incorporate the low-level responses (e.g. ego vehicle speed or acceleration) in the planning loop. Such design might be due to some hardware consideration, but it clearly distinguishes the factory planners from a regular CF model or rule-based controller in the current literature. We point out the differences here and encourage further studies to investigate the impact of these changes on safety or traffic mobility. 

On the other hand, we find the factory ACC planner design is somewhat 'manual', still lacks the base theory and needs more improvement, especially for the MPC planner with hand-crafted cost objectives. For example, the desired distance of the MPC in \eqref{mpc-desireD} is quite different from that in the linear ACC \eqref{desire_d}. The purpose of such desired distance is not straightforward and definitely needs more justifications. The weights for different sub-costs in \eqref{MPC-cost} are often empirically chosen which also needs more theory regarding the safety or SS performance. Future studies are encouraged to work towards this direction. 


By far we have only seen two major types of ACC planners, the linear and MPC controller, which both originate from the control area. It's puzzling that the large body of CF models in traffic flow domain has not been applied or even tested. The paper indicates; see the pipeline in Fig.\ref{pipeline}; any type of models should work if it can output reasonable target speed or acceleration. Thus we strongly encourage future studies to explore the CF models and study their feasibility for commercial ACC products. To assist this, the authors have implemented the well-known Intelligent Driver Model (IDM) in the github repository to replace the role of an linear ACC or MPC. Interested readers are encouraged to replace the IDM model with other CF models and test their performance on commercial cars.
% To assist this, the authors have implemented the famous IDM \citep{treiber2000congested} model in the shared github repository. Interested readers can replace it with other CF models and test them on real cars using the experimental method introduced in Section 4. 
% It is worth noting that the experimental method in Section 4 not only works for testing the low-level control designs, but also facilitates  the novel planners. In the shared github repository, the authors have already implemented the IDM model as an example, readers are encouraged to test more CF models in traffic flow domain. 
    
    
The self-driving industry, including the ACCs, is developing rapidly in recent years. For the ACC technologies, we see a trend \citep{zhou2021review} shifting from the radar-only methods to the vision-assisted or even vision-only approaches. Tesla already started to fully ditch radars and use the pure vision Autopilot \citep{tesla-remove} starting from May, 2021. 
We conjecture more future ACC systems will adopt machine learning models such as the deep neural networks as their longitudinal control planners.
% Current factory ACCs are still the level-2 self-driving systems based on the explicit controllers, but the industry is moving towards the level-5 system rapidly using machine learning methods such as the deep neural networks.
But it is unclear that the SS we achieved on the rule-based ACCs can still hold in neural network models. Current theory of the SS condition only applies to the linear ACC models, the SS in the vision-based machine learning ACC models certainly needs more investigation. Study is ongoing to train the string stable machine learning ACCs, whose results will be included in our sequel paper.    


% This study suggests the following future research directions: i) advanced anti-windup design for the integral term in low-level control; ii) special treatment for grade/curve to improve SS; iii) quantifying the potential "conflict" between a fast low-level controller (benefiting SS) and riding comfort or safety; iv) developing the end-to-end learning-based string-stable planner, which is extendable with other learning-based autonomous driving tasks.


